Relational lattices via duality

The natural join and the inner union combine in different ways tables of a relational database. Tropashko [18] observed that these two operations are the meet and join in a class of lattices-called the relational lattices- and proposed lattice theory as an alternative algebraic approach to databases. Aiming at query optimization, Litak et al. [12] initiated the study of the equational theory of these lattices. We carry on with this project, making use of the duality theory developed in [16]. The contributions of this paper are as follows. Let A be a set of column's names and D be a set of cell values; we characterize the dual space of the relational lattice R(D, A) by means of a generalized ultrametric space, whose elements are the functions from A to D, with the P (A)-valued distance being the Hamming one but lifted to subsets of A. We use the dual space to present an equational axiomatization of these lattices that reflects the combinatorial properties of these generalized ultrametric spaces: symmetry and pairwise completeness. Finally, we argue that these equations correspond to combinatorial properties of the dual spaces of lattices, in a technical sense analogous of correspondence theory in modal logic. In particular, this leads to an exact characterization of the finite lattices satisfying these equations.

==> macros.tex <==
\RequirePackage{color}
\RequirePackage{enumerate}
\RequirePackage{ifthen}
\RequirePackage{comment}

\ifthenelse{\isundefined{\final}}{
  \newcommand{\red}[1]{\textcolor{red}{#1}}
}{
  \newcommand{\red}[1]{}
}


\newcommand{\msl}{meet-semilattice\xspace}
\newcommand{\jsl}{join-semilattice\xspace}
\newcommand{\jzsl}{$(\vee,\bot)$-semilattice\xspace}
\newcommand{\sjsl}{sub-\jsl}
\newcommand{\smsl}{sub-\msl}
\newcommand{\slat}{sub-lattice\xspace}
\newcommand{\TBC}{\red{TO BE CONTINUED}}
\newcommand{\WRONG}{\red{WRONG}\xspace}
\newcommand{\NCPF}{\red{NOT COMPLETE, POSSIBLY FALSE}}
\newcommand{\TBWO}{\red{TO BE WORKED OUT}}
\newcommand{\TODO}[1]{\red{TODO: #1}}
\newcommand{\rto}{\xrightarrow{\quad}}
\newcommand{\set}[1]{\{ #1 \}}
\newcommand{\downset}[1]{\downarrow \!{#1}}
\newcommand{\upset}[1]{\uparrow\!{#1}}
\newcommand{\tiff}{\text{ iff }}
\newcommand{\tssi}{\tiff}
\newcommand{\tand}{\text{ and }}
\newcommand{\tsi}{\text{ if }}
\newcommand{\tst}{\text{ s.t. }}
\newcommand{\semidirect}[1][j]{\ltimes_{#1}}
\newcommand{\sdp}[1][j]{\semidirect[#1]}
\newcommand{\expo}[2]{{#2}^{#1}}
\newcommand{\AD}{\expo{A}{D}}
\newcommand{\BD}{\expo{B}{D}}
\RequirePackage{amssymb}
\newcommand{\restr}[1][]{{\!}_{\restriction_{#1}}}
\newcommand{\rrestr}[1][]{{\!\!}\restriction\!\!\restriction_{#1}}

\RequirePackage{xspace}
\newcommand{\js}{join-semilattice\xspace}
\newcommand{\jirr}{join-irreducible\xspace}
\newcommand{\jr}{join-reducible\xspace}
\newcommand{\cjirr}{completely \jirr}
\newcommand{\jp}{join-prime\xspace}
\newcommand{\jpr}{join-preserving\xspace}
\newcommand{\mpr}{meet-preserving\xspace}
\newcommand{\cjp}{completely \jp}
\newcommand{\njp}{non-\jp}
\newcommand{\jps}{\jp{s}\xspace}
\newcommand{\jirrs}{\jirr{s}\xspace}
\newcommand{\Ji}{\mathcal{J}}
\newcommand{\Jic}{\Ji_\mathtt{c}}
\newcommand{\Jp}{\mathcal{J}_\mathtt{p}}
\newcommand{\jc}{join-cover\xspace}
\newcommand{\mjc}{minimal \jc}
\newcommand{\Mjc}{Minimal \jc}
\newcommand{\ijc}{irredundant \jc}
\newcommand{\mjcing}{\mjc{ing}\xspace}
\newcommand{\mjcings}{\mjcing{s}\xspace}
\newcommand{\jcs}{\jc{s}\xspace}
\newcommand{\ex}{exact\xspace}
\newcommand{\malcev}{Malcev\xspace}
\newcommand{\BC}{Beck-Chevalley\xspace}
\newcommand{\BCp}{\BC property\xspace}
\newcommand{\BCM}{\BC-\malcev}
\newcommand{\BCMp}{\BCM property\xspace}
\newcommand{\Pc}{pairwise complete\xspace}
\newcommand{\Pcs}{\Pc subspace\xspace}
\newcommand{\PC}{\Pc{ness}\xspace}
\newcommand{\PPC}{Pairwise completeness\xspace}
\newcommand{\refines}{\ll}
\newcommand{\wrefines}{\mbox{$\covered\!\!\!\mcovered$}}
\newcommand{\Drefines}{$D$-refines\xspace}
\newcommand{\srefines}{\wrefines}

\newcommand{\covered}{\lhd}
\newcommand{\mcovered}{\covered_{\mathtt{m}}}
\newcommand{\icovered}{\covered_{\mathtt{i}}}
\newcommand{\covers}{\rhd}
\newcommand{\lhs}{left-hand side\xspace}
\newcommand{\rhs}{right-hand side\xspace}
\newcommand{\bv}{\bigvee}
\newcommand{\R}{\mathsf{R}}
\newcommand{\Rl}{\R^{\leq}}
\renewcommand{\L}{\mathsf{L}}
\newcommand{\Ls}{\widehat{\L}}
\newcommand{\dl}{\delta^{\leq}}
\renewcommand{\d}{\delta} 
\newcommand{\dB}{\d_{B}} 
\newcommand{\vv}{\nu} 


\ifthenelse{\isundefined{\lsllncs}}{
\newtheorem{proposition}{Proposition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[proposition]{Lemma}
\newtheorem{corollary}[proposition]{Corollary}
\theoremstyle{remark}
\newtheorem{claim}[proposition]{Claim}
\newenvironment{pofclaim}{\begin{proof}[Proof of Claim.~]}
  {\end{proof}}
\theoremstyle{definition}
\newtheorem{definition}[proposition]{Definition}
\newtheorem{example}[proposition]{Example}
\newenvironment{Example}{\begin{example}}{\qed\end{example}}
\newtheorem{remark}[proposition]{Remark}
\newtheorem{oproblem}{Open problem}
\newtheorem{question}[proposition]{Question}
\newtheorem{conjecture}[proposition]{Conjecture}
\newenvironment{solution}{Solution.~}{\qed\par}
\newenvironment{tsolution}{\noindent{\bf Tentative
    solution.~}}{\qed\par}
\DeclareMathOperator{\card}{card}
}{
\DeclareMathOperator{\card}{card}
}

\newcommand{\pperfect}{pluperfect\xspace}
\newcommand{\apperfect}{almost \pperfect}
\newcommand{\fermentable}{\perfect}

\newcommand{\smalllhs}[2][20mm]{\makebox[#1][l]{$#2$}}
\newcommand{\smallrhs}[2][60mm]{\makebox[#1][r]{$#2$}}
\newcommand{\DNF}{\mathtt{dnf}}

\newcommand{\hy}[1][i]{\widehat{y_{#1}}}

\newcommand{\AxRLone}{\eqref{eq:AxRL1}\xspace}
\newcommand{\AxRLtwo}{\eqref{eq:AxRL2}\xspace}

\newcommand{\RMod}{\eqref{eq:RMod}\xspace}
\newcommand{\Unjp}{\eqref{eq:Unjp}\xspace}
\newcommand{\Unjpp}{\eqref{eq:Unjpp}\xspace}
\newcommand{\Sym}{\eqref{eq:Sym}\xspace}
\newcommand{\SSym}{\eqref{eq:SSym}\xspace}
\newcommand{\SSymBC}{\eqref{eq:SSymBC}\xspace}
\newcommand{\MyAxRLone}{\eqref{eq:MyAxRL1}\xspace}
\newcommand{\SymBC}{\eqref{eq:N1}\xspace}
\newcommand{\None}{\SymBC}
\newcommand{\Dist}{\eqref{eq:Dist}\xspace}

\newcommand{\PSym}{\eqref{prop:Sym}\xspace}
\newcommand{\PSymBC}{\eqref{prop:SymBC}\xspace}
\newcommand{\PJP}{\eqref{prop:JP}\xspace}
\newcommand{\PRMod}{\eqref{prop:RMod}\xspace}
\newcommand{\PMyAxRLone}{\eqref{prop:MyAxRL1}\xspace}

\newcommand{\Dstep}{$D$-step\xspace}
\newcommand{\DSTEP}[3]{#1 \mcovered^{#2} #3}

\newcommand{\macefour}[1][~\cite{prover9-mace4}]{\texttt{Mace4}#1\xspace}

\newcommand{\N}{\mathbb{N}}
\newcommand{\F}{\mathfrak{f}}
\newcommand{\Fe}{\F_{\emptyset}}
\newcommand{\Cl}{\mathtt{Cl}}
\newcommand{\Clos}{\mathtt{Closed}}
\newcommand{\Closed}{\Clos}
\newcommand{\Clop}{\mathtt{Clop}}

\newenvironment{condition}[1][0.1\linewidth]{
  \par\noindent
  \mbox{\hspace{#1}}\begin{minipage}[t]{0.9\linewidth}\em}
  {\end{minipage}}

\DeclareMathOperator{\Ins}{Ins}

\newcommand{\lcd}[1][y]{\mathtt{d}^{o}_{\ell}(\vec{#1})}
\newcommand{\rcd}[1][y]{\mathtt{d}^{o}_{\rho}(\vec{#1})}
\newcommand{\lcdy}{\lcd}
\newcommand{\rcdy}{\rcd}
\newcommand{\lcdz}{\lcd[z]}
\newcommand{\rcdz}{\rcd[z]}

\newcommand{\ld}[1][y]{\mathtt{d}_{\ell}(\vec{#1})}
\newcommand{\rd}[1][y]{\mathtt{d}_{\rho}(\vec{#1})}

\newcommand{\ldy}{\ld}
\newcommand{\rdy}{\rd}
\newcommand{\ldz}{\ld[z]}
\newcommand{\rdz}{\rd[z]}

\newcommand{\POSETS}{\mathsf{Posets}}
\newcommand{\JSL}{\mathsf{SL}_{\vee}}

\newcommand{\pos}[1][\quad]{\langle #1 \rangle}
\newcommand{\compl}{\mathsf{c}}
\renewcommand{\complement}[1]{{#1}^{\compl}}

\newcommand{\JP}[1]{#1}
\newcommand{\JJP}[1]{\widehat{#1}}

\newcommand{\Provern}{\texttt{Prover9}\xspace}
\newcommand{\Macef}{\texttt{Mace4}\xspace}
\newcommand{\Waldmeister}{\texttt{Waldmeister}\xspace}

\newcommand{\myitem}[1]{\bullet\;\;&}

\newcommand{\AXRL}[1][2]{AxRL{#1}\xspace}

\renewcommand{\table}[3][]{
  \bgroup
  \def\arraystretch{1.7}
  \tiny
  \begin{tabular}{|@{\,}#2@{\,}|}
    \hline #3
    \\\hline
  \end{tabular}
  \egroup}
\newcommand{\Pref}[1]{P\ref{P:#1}}
\newcommand{\A}{\mathfrak{A}}


\newcommand{\nj}{natural join\xspace}
\newcommand{\iu}{inner union\xspace}

\newcommand{\Groth}{Grothendieck\xspace}

\newcommand{\HS}{\mathsf{HS}}
\newcommand{\HSP}{\mathsf{HSP}}
\newcommand{\Sub}{\mathsf{S}}
\newcommand{\PU}{\mathsf{P}_{\mathcal{U}}}
\newcommand{\V}{\mathsf{V}}
\newcommand{\si}{subdirectly-irreducible\xspace}
\newcommand{\Hc}{\mathsf{H}_{\texttt{c}}}
\newcommand{\Sc}{\mathsf{S}_{\texttt{c}}}

\newcommand{\cpl}{\mathtt{cpl}}
\newcommand{\Fz}{F_{0}}
\newcommand{\closure}[2][]{\overline{#2}^{#1}}

\newcommand{\Sfive}{\ensuremath{\mathrm{S5}}\xspace}
\newcommand{\sfive}{\Sfive}
\newcommand{\K}{\ensuremath{\mathrm{K}}\xspace}
\renewcommand{\k}{\K}


\newcommand{\Axioms}{[[AxRel]]\xspace}
\newcommand{\RH}{\ensuremath{\Cat{R}^{H}}}
\newcommand{\Frames}{\ensuremath{\Cat{Frames}}\xspace}
\newcommand{\Cat}[1]{\mathsf{#1}}
\newcommand{\U}{\mathfrak{U}}
\newcommand{\FF}{\mathfrak{F}}

\newcommand{\RDA}{\R(D,A)}
\newcommand{\contr}{a contradiction\xspace}
\newcommand{\Bcontr}{By the way of contradiction\xspace}

\newcommand{\LA}{\L^{\!\!A}}

\newcommand{\identity}{equation\xspace}
\newcommand{\prop}{$\pi$-}

\newcommand{\PSSymBC}{\eqref{prop:PSSymBC}\xspace}
\newcommand{\pmorphism}{$p$-morphism\xspace}
\newcommand{\Sec}[1]{\mathsf{Sec}(#1)}

\newcommand{\step}[1][]{ \xrightarrow{#1}}

\newcommand{\END}{\end{document}}
\newcommand{\bpres}{bounds-preserving\xspace}


